Make One-Shot Video Object Segmentation Efficient Again

Video object segmentation (VOS) describes the task of segmenting a set of objects in each frame of a video. In the semi-supervised setting, the first mask of each object is provided at test time. Following the one-shot principle, fine-tuning VOS methods train a segmentation model separately on each given object mask. However, recently the VOS community has deemed such a test time optimization and its impact on the test runtime as unfeasible. To mitigate the inefficiencies of previous fine-tuning approaches, we present efficient One-Shot Video Object Segmentation (e-OSVOS). In contrast to most VOS approaches, e-OSVOS decouples the object detection task and predicts only local segmentation masks by applying a modified version of Mask R-CNN. The one-shot test runtime and performance are optimized without a laborious and handcrafted hyperparameter search. To this end, we meta learn the model initialization and learning rates for the test time optimization. To achieve optimal learning behavior, we predict individual learning rates at a neuron level. Furthermore, we apply an online adaptation to address the common performance degradation throughout a sequence by continuously fine-tuning the model on previous mask predictions supported by a frame-to-frame bounding box propagation. e-OSVOS provides state-of-the-art results on DAVIS 2016, DAVIS 2017, and YouTube-VOS for one-shot fine-tuning methods while reducing the test runtime substantially. Code is available at https://github.com/dvl-tum/e-osvos.

==> figures/algo_and_ablation.tex <==
%!TEX root = ../paper.tex

\begin{figure}[htb]
  % \centering
  \begin{minipage}{0.502\textwidth}
    \input{algorithms/meta_training}
  \end{minipage}
  \begin{minipage}{0.502\textwidth}
    \input{tables/ablation_study}
  \end{minipage}
\end{figure}

==> figures/meta_model.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/meta_model.png}
    \caption{%
    placeholder figure.
    %
    explain model.
    %
    }
    \label{fig:meta_model}
\end{figure}

==> figures/method.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth, height=0.3\textwidth]{figures/method.png}
    \caption{%
    placeholder figure.
    %
    maybe figure on first page.
    %
    explain method and how matching works with online adaptation.
    }
    \label{fig:method}
\end{figure*}

==> figures/swag.tex <==
\begin{figure*}[ht]
    \centering

    \subfloat[blackswan]{
        \label{fig:swag_1}
        \setlength\tabcolsep{0pt}
        \begin{tabular}{c}
            \includegraphics[width=0.24\textwidth]{figures/blackswan_dog_img.png}
            % \vspace{-0.2cm} \\
            \\
            \includegraphics[width=0.24\textwidth]{figures/blackswan_dog_label.png}
        \end{tabular}}
    \subfloat[dog]{
        \label{fig:swag_2}
        \setlength\tabcolsep{0pt}
        \begin{tabular}{c}
            \includegraphics[width=0.24\textwidth]{figures/dog_blackswan_img.png}
            % \vspace{-0.2cm} \\
            \\
            \includegraphics[width=0.24\textwidth]{figures/dog_blackswan_label.png}
        \end{tabular}}
    \subfloat[horsejump-low]{
        \label{fig:swag_3}
        \setlength\tabcolsep{0pt}
        \begin{tabular}{c}
            \includegraphics[width=0.24\textwidth]{figures/horsejump-low_surf_img.png}
            % \vspace{-0.2cm} \\
            \\
            \includegraphics[width=0.24\textwidth]{figures/horsejump-low_surf_label.png}
        \end{tabular}}
    \subfloat[tennis]{
        \label{fig:swag_3}
        \setlength\tabcolsep{0pt}
        \begin{tabular}{c}
            \includegraphics[width=0.24\textwidth]{figures/tennis_bus_img.png}
            % \vspace{-0.2cm} \\
            \\
            \includegraphics[width=0.24\textwidth]{figures/tennis_bus_label.png}
        \end{tabular}}
    \caption{%
        Our~\textit{Blackswan and Dog} (SWOG) data augmentation for four exemplary video frames of the DAVIS-16 dataset.
        %
        Single object sequences are annotated with random objects and their masks to avoid the memorization of the test sets and force the meta learning to learn the optimization.
    }
    \label{fig:swag}
\end{figure*}

==> tables/ablation_and_youtube.tex <==
%!TEX root = ../paper.tex

% \begin{table}[t]
% \parbox[t]{.43\linewidth}{
%     \input{tables/ablation_study}
% }
% \hfill
% \parbox[t]{.56\linewidth}{
%     \input{figures/e-OSVOS-T}
% }
% \end{table}

% \begin{figure}
% \begin{floatrow}
% \ffigbox{%
%   \input{figures/e-OSVOS-T}
% }{%
%   \caption{A figure}%
% }
% \capbtabbox{%
%   \input{tables/ablation_study}
% }{%
%   \caption{A table}%
% }
% \end{floatrow}
% \end{figure}

==> tables/evaluation_davis_17_test_dev.tex <==
%!TEX root = ../supp.tex

\begin{table*}[t!]
    \centering
    \small
    \caption{VOS performance evaluation on the \textbf{DAVIS 2017 validation and test-dev} benchmark.
        %
        We categorize methods by their application of fine-tuning (FT) and post-processing (PP) of the predicted masks and label methods with an ensemble of models with $\dagger$.
        %
        % $\textrm{Ours}^-$: Our model without online adaptation; $\dagger$: An ensemble of models are used.
        %
        The table is ordered by ${\mathcal{J}}\&\mathcal{F}$ on DAVIS 2017 validation.
        %
        The evaluation metrics are detailed in Sec.~\ref{sec:eval_metrics} of the main paper.
    }
    % \vspace{-\baselineskip}
    \resizebox{0.7\textwidth}{!}{
    \begin{tabular}[t]{lcc HHHHH cccc ccccc} 
        \toprule
        &  &  & \multicolumn{5}{H}{DAVIS 2016 - validation} & \multicolumn{4}{c}{DAVIS 2017 - validation} & \multicolumn{4}{c}{DAVIS 2017 - test-dev} \\ 
        %
        \cmidrule(lr){4-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
        %
        Method                              & FT & PP & ${\mathcal{J}} \uparrow$ & ${\mathcal{J}}$ Decay $\downarrow$ & ${\mathcal{F}}\uparrow$ &  ${\mathcal{J}}\&\mathcal{F} \uparrow$ & FPS $\uparrow$ & ${\mathcal{J}}\uparrow$ & ${\mathcal{J}}$ Decay $\downarrow$ & ${\mathcal{F}}\uparrow$ &  ${\mathcal{J}}\&\mathcal{F}\uparrow$ & ${\mathcal{J}}\uparrow$ & ${\mathcal{J}}$ Decay $\downarrow$ & ${\mathcal{F}}\uparrow$ &  ${\mathcal{J}}\&\mathcal{F}\uparrow$\\
        
        \cmidrule(r){1-3} \cmidrule(lr){4-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
        % MaskRNN~\cite{hu2017maskrnn}      & & &$\times$ & 45.5 & --  & -- & -- & 0.60 & --  & -- & -- & -- \\
        FAVOS~\cite{Cheng_favos_2018}        & &$\times$ & 82.4 & \textbf{4.5}  & 79.5 & 80.9 & 0.56 & 54.6 & 14.1  & 61.8 & 58.2 & 42.9 & 18.1 & 44.2 & 43.6 \\ 
        % CTN~\cite{Jang_2017_CVPR}         & & & $\times$  & -- & --  & -- & -- & -- & 73.5  & 15.6 & 69.3 & 71.4 & 1.33 \\  
        % FAVOS~\cite{Cheng_2018_CVPR}      & & &  & -- & --  & -- & -- & -- & 77.9  & -- & 76.0 & 76.9 & 0.60 \\ 
        % VPN~\cite{Jampani_2017_CVPR}      & & &  & -- & --  & -- & -- & -- & 70.2  & 12.4 & 65.5 & 67.8 & 0.63 \\ 
        % BVS~\cite{bvs}                    & & &  & -- & --  & -- & -- & -- & 60.0  & 28.9 & 58.8 & 59.4 & 0.37 \\
        %
        %
        % PML~\cite{Chen_2018_CVPR}             & & &  & -- & --  & -- & -- & -- & 79.3  & 8.5 & 75.5 & 77.4 & 0.27  \\
        % OSMN~\cite{Yang_2018_CVPR}            & & &  & 52.5 & 21.5  & 57.5 & 54.8 & 0.50* & 74.0 & 9.0 & -- & -- & 0.14  \\
        % VideoMatch~\cite{Hu_2018_ECCV}        & & & & 56.5 & --  & -- & -- & 0.35 & 81.0 & --  & -- & -- & 0.32 \\
        RGMP~\cite{oh2018fast}                  & & & 81.5 & 10.9  & 82.0 & 81.7 & \textbf{7.70} & 64.8 & 18.9 & 68.6 & 66.7 & 51.3 & 34.3 & 54.4 & 52.8 \\
        RVOS~\cite{oh2018fast}                  & & & -- & --  & -- & -- & -- & 57.5 & 24.9 & 63.6 & 60.6 & 47.9 & 35.7 & 52.6 & 50.3\\
        % MetaVOS~\cite{meta_words}               & & & 81.5 & 5.0  & 82.7 & 82.1 & 4.0 & 63.9 & 14.4 & 70.7 & 67.3 \\
        RANet~\cite{Ziqin2019RANet}             & & & 86.6 & 7.4 & 87.6 & 87.1 & 30.3 & 63.2 & 18.6 & 68.2 & 65.7 & 53.4 & 21.9 & 57.3 & 55.4\\
        FEELVOS~\cite{voigtlaender2019feelvos}  & & & 81.1 & 13.7  & 82.2 & 81.7 & 2.22 & 69.1 & 17.5 & 74.0 & 71.5 & 55.1 & 29.8 & 60.4 & 57.8\\
        MHP-VOS~\cite{xu2019mhp}                & & & 87.6 & 6.9  & 89.5 & 88.6 & 0.01 & 73.4  & 17.8 & 78.9 & 76.1 & 66.4 & 18.0 & 72.7 & 69.5\\
        STM~\cite{STM_19}                       & & & \textbf{88.7} & 5.0  & \textbf{90.1} & \textbf{89.4} & 6.25 & \textbf{79.2} & \textbf{8.0} & \textbf{84.3} & \textbf{81.7} & \textbf{69.3} & \textbf{16.9} & \textbf{75.2} & \textbf{72.2}\\
        %
        \cmidrule(r){1-3} \cmidrule(lr){4-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
        %
        % MSK~\cite{masktrack}                                                &$\times$ &$\times$ &$\times$ & 79.7 & -- & 75.4 & 77.5 & 0.08 & -- & --  & -- & -- & -- \\
        % MaskRNN~\cite{hu2017maskrnn}                                      &$\times$ & &$\times$ & 60.5 & --  & -- & -- & 9   & 80.7 & --  & 80.9 & 80.8 & 0.60 \\
        % DRL~\cite{Han_2018_CVPR}                                          &$\times$ & & & -- & --  & -- & -- & --  & 84.1 & --  & 84.6 & 84.3 & -- \\
        $\textrm{CINM}^{\dagger}$~\cite{cinm}                               &$\times$ &$\times$ & 83.4 & 12.3  & 85.0 & 84.2 & 0.01 & 67.2 & 24.6 & 74.4 & 70.7 & 64.5 & 20.0 & 70.5 & 67.5\\       
        Lucid~\cite{lucid}                                                  &$\times$ &$\times$ &83.9 & 9.1  & 82.0 & 83.0 & 0.005 & -- & --  & -- & -- & 63.4 & 19.5 & 69.9 & 66.6\\
        % MVOS~\cite{MVOS}                                                &$\times$ &$\times$ & 83.3 & --  & 84.1 & -- & 4.0 & 56.3 & --  & 62.1 & 59.2 \\
        OSVOS~\cite{OSVOS}                                                &$\times$ &$\times$ & 79.8 & 14.9  & 80.6 & 80.2 & 0.11 & 56.6 & 26.1  & 63.9 & 60.3 & 47.0 & 19.2 & 54.8 & 50.9\\
        $\textrm{OSVOS-S}^{\dagger}$~\cite{OSVOS-S}                         &$\times$ &$\times$ & 85.6 & 5.5  & 87.5 & 86.5 & 0.22 & 64.7 & 15.1  & 71.3 & 68.0 & 52.9 & 24.1  & 62.1 & 57.5\\
        OnAVOS~\cite{onavos}                                                &$\times$ &$\times$ & 86.1 & 5.2  & 84.9 & 85.5 & 0.08 & 61.6 & 27.9  & 69.1 & 65.3 & 49.9 & 23.0 & 55.7 & 52.8\\
        
        % ReID~\cite{Li_2018_ECCV}                                            &$\times$ & &$\times$ & -- & --  & -- & -- & --   & 67.3 & -- & 71.0  & 69.1 & 0.43 \\
        $\textrm{PReMVOS}^{\dagger}$~\cite{luiten2018premvos}   &$\times$ & & 84.9 & 8.8  & {\bf 88.6} & {\bf 86.8} & 0.01 & 73.9 & 16.2 & \textbf{81.8} & {\bf 77.8} & \textbf{67.5} & \textbf{21.7} & \textbf{75.8} & \textbf{71.6}\\

        \cmidrule(r){1-3} \cmidrule(lr){4-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
        % e-OSVOS-10                       & $\times$ & & 85.2 & 5.0  & 84.6 & 84.9 & \textbf{4.5} & 69.0  & 15.8 & 75.1 & 72.0 \\
        % e-OSVOS-50                       & $\times$ & & 85.6 & 5.3  & 85.6 & 85.6 & 2.94 & 70.2  & 18.8 & 76.0 & 73.1 \\
        % \cmidrule(r){1-3} \cmidrule(lr){4-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16}
        e-OSVOS-50-OnA                   & $\times$ & & \textbf{86.1} & \textbf{4.4}  & 85.8 & 86.0 & 1.01 & \textbf{74.1}  & \textbf{13.6} & 79.9 & 77.0 & 60.9 & 22.1 & 68.6 & 64.8\\
        \bottomrule
    \end{tabular}         
    }
    %
    \label{tab:evaluation_davis_17_test_dev}
    %
    % \vspace{-\baselineskip}
\end{table*}
